Large-scale Bilingual Language-Image Contrastive Learning

This paper is a technical report to share our experience and findings building a Korean and English bilingual multimodal model. While many of the multimodal datasets focus on English and multilingual multimodal research uses machine-translated texts, employing such machine-translated texts is limited to describing unique expressions, cultural information, and proper noun in languages other than English. In this work, we collect 1.1 billion image-text pairs (708 million Korean and 476 million English) and train a bilingual multimodal model named KELIP. We introduce simple yet effective training schemes, including MAE pre-training and multi-crop augmentation. Extensive experiments demonstrate that a model trained with such training schemes shows competitive performance in both languages. Moreover, we discuss multimodal-related research questions: 1) strong augmentation-based methods can distract the model from learning proper multimodal relations; 2) training multimodal model without cross-lingual relation can learn the relation via visual semantics; 3) our bilingual KELIP can capture cultural differences of visual semantics for the same meaning of words; 4) a large-scale multimodal model can be used for multimodal feature analogy. We hope that this work will provide helpful experience and findings for future research. We provide an open-source pre-trained KELIP.

==> table/tab_english_data.tex <==
\begin{table}[t]
\begin{tabular}{lll}
                      & \# of images & \# of text per image \\
CUB200                &             &                     \\
COCO                  & 118,992     &                     \\
GCC3M                 & 3,318,333	&                     \\
GCC12M                & 12,423,374	&                     \\
YFCC15M               & 14,826,000  &                     \\
WIT                   & 11,400,000  &                     \\
LATION400M            & 413,000,000 &                     \\
Commoncrawl\_2110-2112 & 69,926,360 & 1                   \\
Total                 &             & -                  
\end{tabular}
\caption{English dataset.}
\label{table:english}
\end{table}
